Number Theory and Axiomatic Geometry in the Diproche System

Diproche ("Didactical Proof Checking") is an automatic system for supporting the acquistion of elementary proving skills in the initial phase of university education in mathematics. A key feature of Diproche - which is designed by the example of the Naproche system developed by M. Cramer and others - is an automated proof checker for proofs written in a controlled fragment of natural language specifically designed to capture the language of beginners' proving exercises in mathematics. Both the accepted language and proof methods depend on the didactical and mathematical context and vary with the level of education and the topic proposed. An overall presentation of the system in general was given in Carl and Krapf 2019. Here, we briefly recall the basic architecture of Diproche and then focus on explaining key features and the working principles of Diproche in the sample topics of elementary number theory and axiomatic geometry.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2020 (ThEdu'20)\\
EPTCS 328, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.328.4}{10.4204/EPTCS.328.4}}
\pdfoutput=1

